Retrospective on the 2021 BASALT Competition on Learning from Human Feedback

We held the first-ever MineRL Benchmark for Agents that Solve Almost-Lifelike Tasks (MineRL BASALT) Competition at the Thirty-fifth Conference on Neural Information Processing Systems (NeurIPS 2021). The goal of the competition was to promote research towards agents that use learning from human feedback (LfHF) techniques to solve open-world tasks. Rather than mandating the use of LfHF techniques, we described four tasks in natural language to be accomplished in the video game Minecraft, and allowed participants to use any approach they wanted to build agents that could accomplish the tasks. Teams developed a diverse range of LfHF algorithms across a variety of possible human feedback types. The three winning teams implemented significantly different approaches while achieving similar performance. Interestingly, their approaches performed well on different tasks, validating our choice of tasks to include in the competition. While the outcomes validated the design of our competition, we did not get as many participants and submissions as our sister competition, MineRL Diamond. We speculate about the causes of this problem and suggest improvements for future iterations of the competition.

==> CHANGES <==
v1.29 (2022-01-29):

  * jmlr.cls:

    - added cleveref option

    - fixed draft option

    - bug fix #168: Float-only last pages not counted for page numbering
       https://www.dickimaw-books.com/bugtracker.php?key=168

  * jmlrutils.sty:

    - added cleveref option

    - added \jmlralgorule

    - added \jmlrminsubcaptionwidth

  * jmlrbook.cls:

    - obsoleted (https://www.dickimaw-books.com/faq.php?itemlabel=latex20201009)
      Production editors will need to set the first page number
      of each article manually.

v1.28 (2020-09-21):

  * jmlr.cls:

   Bug fixes: 

    - fixed twoside option (which should be the default)

    - \thanks now uses mpfootnote instead of footnote counter
      with matching \footnotemark and \footnotetext optional
      arguments.

v1.27 (2020-03-26):

  * jmlrutils.sty:

    Bug fix: subfigure and subtable references were producing
    extraneous text (added check for LaTeX kernel version)

v1.26 (2020-01-31):

  * jmlr.cls:

    - removed \vbox from \@jmlrmaketitle to allow for extremely long
      author/affiliation list. Added \ignorespaces before \@author
      to allow for spacing the contents in the code for clarity
      at the start of a long author list.

v1.25 (2020-01-17):

  * jmlr.cls: 

    - Added check for graphics.sty 2019/07/01 (which now detokenizes
      filename)

  * jmlrutils.sty:

    - Added \proofname

v1.24 (2017-08-01):

  * moved non-class related code into new package jmlrutils.sty

  * fixed bug in \includeteximage

v1.23 (2017-03-09):

  * added pmlr class option

v1.22 (2015-04-11):

  * added oneside and twoside class options

v1.21 (2015-02-24):

  * jmlr.cls

    - added check for jmlr2e and pseudocode

    - fixed bug in \thanks to fix footnote marker issue if there's
      more than one \thanks

  * jmlrbook.cls

    - added \nopagebreak after \@editorialteam

v1.20 (2014-10-15):

  * jmlrbook.cls

    - added \jmlrprefaceheader, \jmlrlocation

v1.19 (2014-09-29):

  * jmlrbook.cls

    - changed \chapter* to \chapter in preface environment

v1.18 (2013-10-17):

  * jmlrbook.cls

    - patched to work with auxhook

    - added draft and final options

    - add \booklinebreak

  * jmlr.cls

    - Added calc and etoolbox as required packages

    - Added draft and final options and removed \ds@draft

    - Added starred version of \newtheorem

    - Added \theorembodyfont, \theoremheaderfont, \theorempostheader
      and \theoremsep

v1.17 (2012-05-30):

  * jmlr.cls

    - added \titletag

    - added warnings if obsolete font commands (such as \bf) used

  * jmlrbook.cls

    - added 'articlet' page style

    - \importarticle sets title page style to articlet

    - \importpaper disables \jmlryear, \jmlrworkshop, \jmlrvolume
      and \jmlrissue

    - html title page uses jmlrvolume instead of volume

    - added optional argument to \logo

v1.16 (2012-05-15):

  * jmlr.cls

    - added \@post@hyperref hook

  * jmlrbook.cls

    - added code to deal with \c@lenddoca clash

v1.15 (2012-05-12):

  * jmlrbook.cls

    - added 'algocf' and 'definition' counters to reset list in
      \zeroextracounters

    - added \theHalgocf

    - removed dependence on \ps@headings in \ps@jmlrbook

    - added \markleft

v1.14 (2012-04-24):

  * jmlrbook.cls

    - modified \jmlrwritepdfinfo to write book author and title
      information to aux file
    - fixed bug in fetching time zone information

v1.13 (2012-02-25):

  * jmlrbook.cls

    - added pdfxa option
    - added \jmlrwritepdfinfo
    - changed preface environment to use \chapter* instead of \chapter

  * jmlr.cls

    - added \@pre@hyperref hook

v1.12 (2012-01-05):

  * jmlr.cls

    - removed prehyperref package option.

    - renamed \jmlr@prehyperref to \jmlrprehyperref

    - added tabularx to list of problem packages.

    - provided default value of \@shortitle

    - added \titlebreak

    - added optional argument to \Name
      (\jmlrauthors now redefines \@jmlr@authors instead of
      \@jmlrauthors)

    - added chapter number to \theHsection to ensure unique
      hyperlinks in book

  * jmlrbook.cls

    - Moved loading setspace and fink before jmlr.cls loaded

    - changed \thechapter to \theHchapter in definition of
      \theHalgorithm etc

    - added \theHfootnote, \theHtable, \theHfigure

    - in \importpubpaper etc, changed \@shortitle to \@title in toc

  * makejmlrbook v0.31

    - footnotes in abstract files changed to in-line parentheses.

    - --batchtex option now also passes "-interaction=batchmode" to
      htlatex

    - added debugging option --noexecute

v1.11 (2011-03-24):

  * jmlr.cls

    - fixed typo: WC\&P -> W\&CP

    - added \jmlrabbrnamelist (used by makejmlrbook)

  * jmlrbook.cls

    - now requires fink package

    - added preface environment and \prefacename

    - added algorithm2e old commands (in case some authors are using
      an older version).

  * makejmlrbook (v0.3):

    - added changes made by Olivier Chapelle to add JMLR menu on the
      left side of the page and use description environment for each
      paper of the TOC.

    - added --extractpreface option

    - set hyperref draft mode for abstract only html pages.

    - abstract html source files now input original aux files to allow
      for citations.

v1.10 (2011-01-05):

  jmlr.cls

  * now loads xkeyval

  * now loads hyperref (instead of jmlrbook loading it)

  * added class option prehyperref={stuff to do before hyperref loaded}

  * added class option tablecaption=<position> (where <position> can
    either be top or bottom).

  * fixed 10pt, 11pt and 12pt class options, which weren't having
    any effect.

  * modified \thanks to ensure hyperlink works correctly.

  * added \mdseries to definition of \addr.

  * added \startpage (used by jmlrmakebook).

  * modified \artpart and \bookpart to correct bookmark level number

  jmlrbook.cls

  * code loading hyperref moved to jmlr.cls

  * added 10pt, 11pt and 12pt class options.

  * Removed redundant redefinition of \@bookpart

  makejmlrbook (v0.2):

  * Uses \startpage to set initial page number for stand-alone 
    articles.

  * Makes subdirectories in html directory for each article.

  * copies any image files generated by tex4ht into html directory.

  * added time stamp at the end of each of the generated html file.

v1.09 (2010-12-01):

  jmlr.cls

  * now loads article.cls instead of scrartcl.cls

  * Fixed sub-captions so that they don't exceed the width of the
    sub-figure/table to which they refer.

  * added \nametag, \reprint, \algocfconts, \theHsubfigure,
    \booktocpreamble, \@partapp.

  * Made \objectref robust

  jmlrbook.cls

  * Reset start and end document hook to avoid problems caused by
    defining duplicate commands.

  * Moved redefinition of \jmlrpremaketitlehook outside of import
    macros.

  * Moved \refstepcounter from \jmlrmaketitlehook to
    \jmlrpremaketitlehook

  * Added \jmlrimporthook

  * Added \label to \jmlrmaketitlehook

v1.08 (2010-07-27):

  * Fixed \thanks so that the footnote symbol is raised and isn't
    followed by a full stop.

v1.07 (2010-06-30):

  * Added check for two column

v1.06 (2010-06-17):

  jmlr.cls

  * Added tablecaptiontop and tablecaptionbottom class options

v1.05:

  jmlrbook.cls

  * Added \productioneditors

v1.04:

  * Added Perl script makejmlrbook

  jmlrbook.cls

  * Added patch to fix references in print mode

  * Added code to work with makejmlrbook

  jmlr.cls

  * Added code to work with makejmlrbook

v1.03:
  jmlrbook.cls

  * Added patch to combnat

  jmlr.cls

  * Added \editors, \editorname and \editorsname

v1.02:
  jmlrbook.cls:

  * Added \issue

  jmlr.cls

  * Added \jmlrissue

v1.01 :

  jmlrbook.cls: 

  * added \importpaper

  * added \titlebody, \SetTitleElement and \IfTitleElement to 
    make it easier to customise the front page of the book.

  jmlr.cls:

  * fixed the last page anchor.

v1.0 : Initial release

